Neural apparent BRDF fields for multiview photometric stereo

We propose to tackle the multiview photometric stereo problem using an extension of Neural Radiance Fields (NeRFs), conditioned on light source direction. The geometric part of our neural representation predicts surface normal direction, allowing us to reason about local surface reflectance. The appearance part of our neural representation is decomposed into a neural bidirectional reflectance function (BRDF), learnt as part of the fitting process, and a shadow prediction network (conditioned on light source direction) allowing us to model the apparent BRDF. This balance of learnt components with inductive biases based on physical image formation models allows us to extrapolate far from the light source and viewer directions observed during training. We demonstrate our approach on a multiview photometric stereo benchmark and show that competitive performance can be obtained with the neural density representation of a NeRF.

==> old/litreviewbackup.tex <==

\subsection{Neural 3D Representations}

Previous works in the field of neural rendering have learned shape priors from partial or noisy data. Local Implicit Grid Representations \cite{4} trains an autoencoder to handle complex and diverse indoor scenes. Continuous Single Distance Function (DeepSDF) \cite{5} provides trade-offs across fidelity, efficiency and compression capabilities enabling high quality shape representation, interpolation and completion. Local Deep Implicit Functions (LDIF) \cite{6} and Occupancy Networks \cite{7} provide a computationally efficient function for high-resolution geometry representation for arbitrary topology. However, these representation functions are limited by a major factor – they all require access to ground truth of the 3D geometry which is typically obtained from a synthetic 3D shape.

\medskip

A step up from these techniques have been in training reconstruction models from RGB images, however, these approaches have been restricted to voxel- \cite{9, 10, 11} and mesh-based \cite{12, 13, 14, 15} representations which suffer from discretization or low resolution \cite{8}. Recent works have provided a rather relaxed dependency on ground truth 3D geometry and essentially employing only 2D images to formulate differentiable rendering functions. Niemeyer \etal \cite{8} propose to learn implicit shape and texture representations using depth gradients which are derived from implicit differentiation. This is obtained by calculating the surface intersection for each ray which is the input to a neural 3D texture field predicting a diffuse colour at a particular point. Sitzmann \etal \cite{16} propose Scene Representation Networks (SRNs) which provides a structure-aware scene representation through a continuous function mapping world coordinates to features of a local scene – achieved through a differentiable ray-marching algorithm. These techniques have quite a potential to represent complicated and high-resolution geometry, they are still limited to extremely low geometric complexity leading to oversmoothed renderings.

\subsection{View Synthesis and Image-based Rendering}

Photorealistic novel views can be reconstructed when the data sampling is dense in nature by widely popular interpolation techniques, however, when the sampling is sparse in nature it becomes difficult to predict geometry and appearances from observed images. Multiple approaches have been developed to address this problem – most popular being mesh-based and volumetric representations \cite{1}. 

\medskip

Mesh-based representations can be directly optimized using differentiable rasterizers and pathtracers. DIB-R \cite{17} implements a differentiable renderer which views foreground rasterization as a weighted interpolation of local properties and background rasterization as a distance-based aggregation of global geometry – which, in turn, enables gradient calculation for all pixels in the image. Similarly, soft rasterizers \cite{18} renders using an aggregation functions which collates probabilistic contributions of all mesh triangles with respect to the rendered pixels. Monte Carlo ray tracer \cite{19} through edge sampling provides a comprehensive solution to calculate scalar function derivates over a rendered image with respect to parameters like camera poses, lighting and scene geometry. However, these strategies require a template mesh with a fixed topology which is not possible for in-the-wild scenes.

\medskip

Volumetric representations provide superior reconstruction for complex shapes and materials as they can be easily optimised through gradient-based approaches and are less prone to visually distracting artefacts. Modern approaches generally use large scene datasets which train over deep networks to predict volumetric representations and render novel views using alpha- or custom composting. DeepView \cite{20} synthesises multiplane images (MPI) from sparse camera viewpoints improving performance on object boundaries, light reflection and thin structures. Local light field fusion (LLFF) \cite{21} proposed an algorithm by extending the traditional plenoptic sampling theory for view synthesis from an irregular grid of sample views via MPI representations. Neural Volumes \cite{22} present an encoder-decoder framework which outputs a 3D volume representation from images and a differentiable ray-marching operation for end-to-end training. Though, these techniques have potential to high resolution novel view points, yet they are limited due to discrete sampling. 

\subsection{Neural Radiance Fields}
The field of Neural Field Radiance has received significant attention due to their impressive results in capturing unbounded and bounded 360 degree scenes.  While NeRF works well on images of static subjects captured under controlled settings, it is incapable of modelling many ubiquitous, real-world phenomena in uncontrolled images, such as variable illumination or transient occluders \cite{33}. NeRF++ \cite{23} applies NeRF to 360 degree, large-scale, unbounded 3D scenes by applying shape radiance ambiguity and creating inverted sphere parameterization - separately modelling foreground and background. NeRF-W \cite{33} introduces a system for 3D reconstruction from in-the-wild photo collections. This was achieved by introducing Generative Latent Optimization (GLO) \cite{34} - making the approximation with respect to image-dependent radiance - and modelling observed colour as a probability distribution (isotropic normal distribution) over its value.  

\medskip

Deformable NeRFs \cite{35} presents a method for photorealistic reconstruction of a non-rigidly deforming scene from casually captured photos and videos from mobile phones - 'nerfies'. It presents multiple techniques to improve robustness - coarse-to-fine optimization and elastic regularization of deformed fields. Though vanilla NeRF is applicable to static scenes, D-NeRF \cite{36} extends the applicability to dynamic domain which allows reconstruction and rendering of objects under motion from a single moving camera. The time varying deformation is performed through two modules - one learning a canonical configuration and other learning the displacement field with respect to the canonical space. Another extension into the dynamic domain is Neural Scene Flow Fields \cite{37} which models dynamic scenes as a time-variant continuous function of appearance, geometry and 3D scene motion. Neural Irradiance Fields \cite{38} enables rendering of video from novel viewpoints. 

\medskip

A fundamental obstacle to making these methods practical is the extreme computational and memory requirements caused by the required volume integrations along the rendered rays during training and inference \cite{31}. DeRF \cite{29} presents a solution to NeRF's computationally intensive nature using spatial decomposition where each portion of the scene is handled by smaller networks which can work together to render the complete scene. Furthermore, employing Voronoi spatial decomposition is efficient for GPU rendering and thus DeRF's inference is 3 times more efficient than NeRF. It also circumvents the issue of diminishing returns in neural rendering. Neural Sparse Voxel Fields (NSVF) \cite{30} provided faster (20x) and high quality free-viewpoint rendering using voxel-bounded implicit fields. These model local properties of each cell by learning the underlying voxel structure - using a differentiable ray-marching operation - and skipping ones which do not provide any scene content. AutoInt \cite{31} presents an efficient learning framework using implicit neural networks. When applied to neural volume rendering, it provides improved computational efficiency. 

\medskip

Generative Radiance Fields (GRAF) \cite{32} present a generative model with multi-scale patch-based discriminator which demonstrates synthesis of high-resolution results from unposed 2D images. The discriminator is implemented as a convolutional neural network which compares the predicted patch to a patch extracted from a real image. The framework generates higher resolution images from voxel-based approaches but is limited to simple scenes with single objects - incorporating inductive biases could extend it to real world images.

\medskip

Neural Reflectance Decomposition (NeRD) \cite{59} presents a model which decomposes a scene into its shape, reflectance and illumination. A scene's decomposition into explicit representations leverages any rendering framework to generate novel views under any illumination in real-time. NeRD achieves this by introducing physically-based rendering to vanilla NeRF \cite{1}. Building on the NeRF's Multi-Layer-Perceptrons, NeRD's architecture differs specifically in the finer network - by using light independent reflectance parameters instead of direct view-dependent colour. The bidirectional reflectance distribution function (BRDF) is estimated using additional network which creates severe bottleneck i.e. a two-dimensional latent space encoding every possible BRDFs in the scene. As the underlying shape and BRDF are preemptively assumed to be same for all the views, the model converges to a consistent state for input images with varied illumination. Neural Reflectance and Visibility Fields (NeRV) \cite{58} describes a model which can render a 3D representation for novel viewpoints under arbitrary lighting conditions from a set of input images with unconstrained known lighting conditions. It takes 3D location as input to learn scene properties like volume density, surface normal, material parameters, distance to the first surface intersection and visibility of external environment in any direction. Altogether, they not only provide novel views but also indirect illumination effect which makes the model's performance superior to prior approaches.

With the advent of Neural Radiance Fields, neural networks can now render novel views of a 3D scene with quality that fools the human eye \cite{29}. Yet, multiple open challenges are present in order to faithfully attain photorealism for bounded and unbounded scenes. 

\medskip

\noindent\textbf{Technique drawbacks:} Training and testing of NeRF is memory intensive and time consuming. Liu \etal \cite{30} have though provided techniques to speed up inference, but rendering is still time consuming. The method is unable to handle scenes with complex backgrounds. Camera calibration are very sensitive - a minor error leads NeRF to failure. Image fidelity could be improved by taking photometric effects into consideration \cite{23}.  The model learns colour and density as a 'black-box' function of query point location and camera-ray direction \cite{1, 16, 30} which makes it highly dependent on training image quality and distribution which may produce artefacts. Existing methods either produce low image resolution or fall short in disentangling camera and scene properties, e.g., the object identity may vary with the viewpoint \cite{32}. These factors limit their applicability in practical scenarios.

\medskip

\noindent\textbf{Scope:} Robustness and generalisation can be improved by incorporating traditional radiance and rendering equations as an inductive bias to the neural network models. Furthermore, state-of-the-art techniques require known camera poses as input for initializing rays and their directions. These are quite prone to camera calibration errors and difficult to achieve for real images. Future research directions could look into unsupervised techniques (like GANs) for prediction of camera poses for such data \cite{30}. Deformable NeRF \cite{35} has extended NeRF by modelling non-rigigdly deformed scenes, however, these can be extended to models handling large deformations and to static camera captures under variable light where lighting changes could help in recovery of object geometry. Though NeRF-W \cite{33} is able to synthesis photorealistic and temporally consistent rendering from unstructured photos, the problem of outdoor scene reconstruction is far from being fully solved. 

\medskip

\noindent\textbf{Technique: Neural Representation through NeRF:} \label{nerf}
The technique addresses the view synthesis problem through parameter optimization of a 5D scene representation so as to minimize the error of rendering a set of captured images. The input 5D representation consists of three spatial coordinates $(x,y,z)$ and viewing directions ($\theta,\phi$). The network encompasses a deep fully connected neural network without any convolutional layers (Multilayer Perceptron MLP). The network outputs the radiance emitted in each direction at each point in space along with a density at each point which acts like a differential opacity controlling the amount of radiance which is accumulated when it passes through a particular point \cite{1}. Previously, such MLP architectures have been used to represent natural textured materials which can be sampled over infinite domains \cite{2} or circumvent factors – like in Texture Fields – which limit the fidelity of highly textured surfaces \cite{3}. 

\medskip

A continuous scene is represented as a 5D vector function with inputs 3D location $\mathbf{x} = \mathbb{(x, y, z)}$ and 2D viewing direction $\mathbb{(\phi,\theta)}$ which outputs an emitted colour $\mathbf{c}=\mathbb{(r,g,b)}$ and volume density $\mathbb{\sigma}$. The direction is represented as a 3D Cartesian unit vector $\mathbf{d}$ and the scene then can be approximated with an MLP network $\mathbb{F_{\Theta}: (\mathbf{x,d})\rightarrow(\mathbf{c,\sigma})}$. The network optimises weights $\Theta$ so as to map from each input 5D coordinate to its respective volume density and directional emitted colour. The volume density function $\sigma$ is restricted to be a function of location $\mathbf{x}$ in order to maintain multiview consistency. 

\medskip

\noindent \textbf{Volume Rendering}
Using the principles of classical volume rendering \cite{54}, the colour of any ray passing through a scene can be rendered. It states that the volume density $\mathbb{\sigma}(\mathbf{x})$ can be expressed as the differential probability of a ray terminating at an infinitesimal particle at location $\mathbf{x}$, then the expected colour $\mathbb{C}(\mathbf{r})$ of camera ray $\mathbf{r}\mathbb{(t)}=\mathbf{o}+\mathbb{t}\mathbf{d}$ with near and far bounds $\mathbb{t_{n}}$ and $\mathbb{t_{f}}$ is

\begin{equation}
    \mathbb{C(\mathbf{r})}=\int_{t_n}^{t_f} T(t)\sigma(\mathbf{r}(t))\mathbf{c}(\mathbf{r}(t),\mathbf{d})dt \\
\end{equation}

where
\begin{equation}
    T(t)=\mathrm{exp}\left(-\int_{t_n}^{t}\sigma(\mathbf{r}(s))ds\right).
\end{equation}

The function $\mathbb{T(t)}$ represents the accumulated transmittance along the ray from $t_n$ to $t$ which is the probability of the ray travelling from $t_n$ to $t$ without hitting any other particle. This continuous integral is estimated using stratified sampling where $[t_n, t_f]$ is divided into $N$ evenly-spaced bins and values are randomly sampled from each bin as

\begin{equation}
    t_i\sim \mathcal{U}\left[t_n + \frac{i-1}{N}(t_f-t_n), t_n+\frac{i}{N}(t_f-t_n) \right]
\end{equation}

These samples are used to estimate $\mathbb{C}(\mathbf{r}$) with the quadrature rule \cite{55} as

\begin{equation}
    \hat{C}(\mathbf{r})=\sum_{i=1}^{N}T_i(1-\mathrm{exp}(-\sigma_i\delta_i))\mathbf{c}_i,
\end{equation}

where
\begin{equation}
    T_i = \mathrm{exp}\left( -\sum_{j=1}^{i-1}\sigma_j\delta_j\right),
\end{equation}

where $\delta_i=t_{i+1}-t_i$ is the distance between adjacent samples and $\alpha_i=1-\mathrm{exp}(-\sigma_i\delta_i)$ represents alpha composting.

\medskip

\noindent \textbf{Optimisation}
Volume rendering alone proves insufficient for achieving state-of-the-art rendering quality. The quality of complex scene representation in NeRF can be attributed to two factors - positional encoding and hierarchical volume sampling.

\begin{itemize}
    \item \underline{Positional Encoding:} It has been observed that the network $F_\Theta$ performs sub par when representing high-frequency variations in colour and geometry which can be attributed to deep networks being biased towards learning lower frequency functions \cite{56}. Therefore, operating on $xyz\theta\phi$ require working with a composite function $F_\Theta=F_\Theta^{'}\circ\gamma$ ($\gamma$ is a mapping from $\mathbb{R}$ into higher dimensional space $\mathbb{R}^{2L}$) so as to enable MLP to more easily approximate a higher frequency function \cite{1}. $\gamma$ is defined as
    
    \begin{equation}
        \gamma(p)=(\sin{(2^0\pi p)}, \cos{(2^0\pi p)},\cdots ,\sin{(2^{L-1}\pi p)}, \cos{(2^{L-1}\pi p)}).
    \end{equation}
    
    \item \underline{Hierarchical Volume Sampling:} Evaluating the network at $N$ query points along every camera ray is computationally intensive and thus inefficient. For a more efficient evaluation, the rendering strategy \cite{57,1}, simultaneously optimises two networks - 'coarse' and 'fine'. A set of $N_c$ locations are used to first compute the 'coarse' network. The output helps in informed sampling of relevant points for further detailed computation. The sole alternation is reconfiguration of alpha composting colour from coarse network as
    \begin{equation}
        \hat{C}_c(\mathbf{r})=\sum_{i=1}^{N_c} w_i c_i, \; \; w_i=T_i(1-\mathrm{exp}(-\sigma_i\delta_i).
    \end{equation}
    \item \underline{Loss Function:} The loss function is defined  as the total squared error between the rendered and true pixel colours for both coarse and fine renderings:
    \begin{equation}
        \mathcal{L}=\sum_{\mathbf{r}\in\mathcal{R}}\left[
        \begin{Vmatrix} 
            \hat{C}_c(\mathbf{r})-C(\mathbf{r})
        \end{Vmatrix}_2^2 +
        \begin{Vmatrix}
            \hat{C}_f(\mathbf{r})-C(\mathbf{r})
        \end{Vmatrix}_2^2\right]
    \end{equation}
    where $\mathcal{R}$ is the set of rays in each batch, and $\hat{C}(\mathbf{r})$, $\hat{C}_c(\mathbf{r})$, and $\hat{C}_f(\mathbf{r})$ are the ground truth, coarse volume predicted, and fine volume predicted RGB colours for ray $\mathbf{r}$ respectively.
\end{itemize}

NeRF \cite{mildenhall2020nerf} -\textgreater{} extensions (focussing on relightable)

Neural reflectance fields for appearance acquisition \cite{bi2020neural}
\medskip

NeRFactor \cite{zhang2021nerfactor}
\medskip

Neural Radiance Factorization (NeRFactor) \cite{zhang2021nerfactor} addresses the issue of recovering the shape and spatial-varying reflectance of an object from multi-view images of an object illuminated by unknown lighting condition which enables the rendering of novel views of the object under arbitrary environment lighting and object's material properties. The major technical contribution include, a method for factorizing images of an object under an unknown lighting condition into shape, reflectance and illumination i.e. creating free-view point relighting (with shadows) and material editing, a strategy to distill NeRF-estimated volume density into surface geometry to use for initialisation and novel data-driven BRDF prior learned from training a latent code model on real measured BRDFs.

\medskip

The input for the NeRFactor model are multi-view images (and their camera positions) of an object lit by an unknown illumination condition. After optimization, NeRFactor outputs, $\mathbf{x}$, a 3D location on the object surface, $\mathbf{n}$ surface normal, $\mathbf{v(\omega_i)}$ light visibility in any direction, $\mathbf{a}$ albedo and $\mathbf{z_{BRDF}}$ reflectance.. By explicitly modeling light visibility, NeRFactor is able to separate shadows from albedo and synthesize realistic soft or hard shadows under arbitrary lighting conditions. NeRFactor is able to recover convincing 3D models for free-viewpoint relighting in this challenging and under constrained capture setup for both synthetic and real scenes.

\medskip

NeRV \cite{srinivasan2021nerv}
\medskip

The Neural Reflectance and Visibility Fields (NeRV) \cite{srinivasan2021nerv} provides a method to render 3D representation of any scene from a novel viewpoint under arbitrary lighting conditions. The NeRV architecture takes 3D locations as input and provides multiple scene properties like volume density, surface normal, material parameters, distance to the first surface intersection in any direction, and visibility of the external environment in any direction. These parameter are crucial for the illumination performance of the model.

\medskip

The NeRF architecture has been enhanced such that instead of modeling a scene as a continuous 3D field of particles which could absorb and reflect light from external source which is unable to scale to simulate realistic lighting condition or global illumination. They introduced a neural visibility field which effectively query the point-to-light and point-to-point visibilities that are required to simulate light transportation. 

\medskip

Relightable NeRF is possible if the representation of a scene is performed using a field of particles that reflect incoming light instead of emitting light. Using this, any arbitrary lighting condition can transport light through the given volume as it is reflected by particles until it reaches the camera with a standard volume rendering integral.

\begin{equation}
    {L(\mathbf{c,\omega_o})}=\int_{0}^{\infty}
    V(\mathbf{x}(t))\sigma(\mathbf{x}(t))L_r(\mathbf{x}(t),\mathbf{\omega_o})dt, \\
\end{equation}

\begin{equation}
    {L_r(\mathbf{c,\omega_o})}=\int_{S}^{}
    L_i(\mathbf{x,\omega_i})R(\mathbf{x,\omega_i,\omega_o})d\mathbf{\omega_i} \\
\end{equation}

where the view-dependent emission is replaced with an integral over the sphere $S$ of incoming direction, which is the product of incoming radiance $L_i$ from any direction and a reflectance function $R$, which describes the amount of light arriving from direction $\omega_i$ and reflected towards direction $\omega_o$.

NeRV implementation has replaced NeRF's radiance MLP with two MLPs: a "shape" MLP which outputs volume density $\sigma$ and a "reflectance" MLP which outputs BRDF parameters (3D diffused albedo \mathbf{a} and one-dimensional roughness $\gamma$) for any input 3D point. Furthermore, they have introcued a "visibility" MLP for estimating general lighting scenarios (which is computationally challenging) which emits an approximation of the environment lighting visibility at any input location along any direction. The approximations are represented as:

\begin{equation}
    {V(\mathbf{x,\omega})}=\exp{\left(-\int_{0}^{\infty} \sigma(\mathbf{x}+s \mathbf{\omega})ds \right)} \\
\end{equation}

% \begin{equation}
%     D(\mathbf{x,\omega})=\int_{0}^{\infty}
%     \exp{\left(-\int_{0}^{t} \sigma(\mathbf{x}+s \mathbf{\omega})$ds$ \right)}$t$\omega(\mathbf{x}+$t$\mathbf{\omega})$dt$
% \end{equation} - I was not able to make this work

\medskip

NeRD \cite{boss2020nerd}
\medskip



\medskip

Object-centric Neural Scene Rendering \cite{guo2020osf}
\medskip

NeRF-W \cite{martinbrualla2020nerfw}
\medskip

NeRF for multi-view stereo, WACV 2022 paper: \url{https://arxiv.org/pdf/2110.05594.pdf}
\medskip

NeRF in the dark (high dynamic range)
% There's a paper appearing at WACV that uses NeRFs for multiview photometric stereo. Thankfully, they're not doing what we're trying to do! Instead, they have a separate network for doing single deep photometric stereo, then inject the normals into the NeRF. I believe our approach is simpler (just the single NeRF network) and more elegant.
% But it's incredibly useful in terms of finding related papers and seeing how they conduct their evaluation and what their baselines are. It also gives us a benchmark performance to aim at. Paper is here: https://arxiv.org/pdf/2110.05594.pdf

\url{https://lioryariv.github.io/idr/}? (NeurIPS 2020)
\medskip

Classical methods for multiview photometric stereo

Key point to make: original NeRF conditioned on x,y,z position (i.e. only input is view direction) is modelling a slice of the apparent BRDF. This captures local (BRDF) shading effects but also some global effects like light dependent shadowing. But all this is baked in and can't be disentangled or modelled.

Objectives: relightable, reconstruct objects where we don't have fixed light for all images (diligent turntable is an example), fully disentangle lighting/reflectance/geometry/camera, give physical meaning to parameters, extrapolate beyond observed lighting conditions, avoid expensive ray casting operations for shadows etc -> solution = model full apparent BRDF with physically meaningful parameters and imposing physical constraints where possible.

Simplest thing to do is simply add lighting dependency to a NeRF, in the same way as viewpoint dependency. In this case, second half of network acts like full apparent BRDF. But without any physical constraints, it can't extrapolate. If it never gets to observe self shadowing for example, it won't learn it (we will compare against this baseline later - it's the first relightable version that Meghna implemented).

